mRI: Multi-modal 3D Human Pose Estimation Dataset using mmWave, RGB-D, and Inertial Sensors

The ability to estimate 3D human body pose and movement, also known as human pose estimation (HPE), enables many applications for home-based health monitoring, such as remote rehabilitation training. Several possible solutions have emerged using sensors ranging from RGB cameras, depth sensors, millimeter-Wave (mmWave) radars, and wearable inertial sensors. Despite previous efforts on datasets and benchmarks for HPE, few dataset exploits multiple modalities and focuses on home-based health monitoring. To bridge the gap, we present mRI, a multi-modal 3D human pose estimation dataset with mmWave, RGB-D, and Inertial Sensors. Our dataset consists of over 160k synchronized frames from 20 subjects performing rehabilitation exercises and supports the benchmarks of HPE and action detection. We perform extensive experiments using our dataset and delineate the strength of each modality. We hope that the release of mRI can catalyze the research in pose estimation, multi-modal learning, and action understanding, and more importantly facilitate the applications of home-based health monitoring.

==> files/intro_backup.tex <==
\section{Introduction}

% thesis statement: what is HPE
Human pose estimation~(HPE) refers to detecting and tracking human body parts or key joints, such as wrists, shoulders, and knees. It is a fundamental and crucial task in vision and human modeling with numerous application areas, including rehabilitation, professional sports, augmented/virtual reality, and autonomous driving~\cite{simon-al-araji_2019, odemakinde_2021, vakanski2018data}. %}
% thesis statement: HPE can be done using multi-modalities
%\statement{
Current practice relies heavily on processing RGB frames from color cameras for human pose \todo{estimation~\cite{}.} 
RGB image and video frames are the most common input types since they offer accurate real-world representations with true color. However, the frame quality depends heavily on the environmental setting, such as light conditions and visibility~\cite{an2021mars}. 
Moreover, using image and video data poses significant privacy and security concerns, especially in home environments. 
Finally, the data-intensive nature of real-time video processing requires computationally powerful equipment with high cost and energy consumption.


Frame quality, privacy, and computational power drawbacks of video processing can be addressed by emerging \textit{complementary sensor modalities}, such as and lidar, millimeter wave~(mmWave) radar~\cite{an2021mars, xue2021mmmesh, zhao2018rf}, and inertial sensors~\cite{vonMarcard2018,von2018recovering,von2017sparse}, 
%signals also show great potential and unique advantages in this domain. %}
The lidar point cloud %, obtained by laser scanning, 
overcomes frame quality and privacy challenges. However, it has a high cost and computation power requirements to process the data, making it unsuitable for indoor applications such as rehabilitation. 
In contrast, mmWave radar can generate high-resolution 3D point clouds of objects while maintaining low cost, privacy, and computational power advantages. 
Similarly, wearable inertial sensors provide accurate rotation and acceleration information regarding joints independent of poor environmental settings with low cost and computational power requirements~\cite{von2017sparse, von2018recovering, vonMarcard2018}. 
Therefore, this work, mRI, combines \underline{m}mWave radar, \underline{R}GB-Depth (RGB-D), and \underline{I}nertial sensors to exploit their complementary advantages. 

%The downside of inertial sensors is that users often refuse to wear additional equipment due to their clumsiness, especially with multiple parts. 

% human3.6: ionescu2013human3, MPII: andriluka20142d, COCO:lin2014, NTU:shahroudy2016ntu, CMU: Joo_2015_ICCV, 3DHP: mono-3dhp2017, 3DPW: von2018
\statement{High quality and large scale datasets are the vital foundation of algorithms development. It is a trend for human pose estimation datasets to include multiple mainstream modalities.} COCO~\cite{lin2014microsoft} and MPII~\cite{andriluka20142d} are two early large-scale human pose estimation datasets with 2D human keypoints annotations. 
% COCO is highly concentrated on object detection, captioning, and segmentation-based data features. Moreover, more than 2,50,000 people's images are annotated with keypoints for pose estimation tasks. MPII consists of around 25K images, including about 40K people with 2D human keypoints annotations. 
However, they only have 2D human keypoints annotations since 2D HPE was a more important task. 
With the development of computation power and 3D HPE algorithms, more datasets with 3D human keypoints annotations are released~\cite{ionescu2013human3, shahroudy2016ntu, Joo_2015_ICCV, mono-3dhp2017} and most of them~\cite{ionescu2013human3, shahroudy2016ntu, Joo_2015_ICCV} also contain the depth frame as the supplementary sensing modalities. 
% As its name implies, Human3.6M~\cite{ionescu2013human3} has 3.6 million 3D human pose images of 11 professional actors on 17 daily activities. High-resolution RGB video frames and depth frames were captured using calibrated and time-of-flight-based four cameras. CMU Panoptic~\cite{Joo_2015_ICCV} is a dataset containing 65 sequences (5.5 hours) and 1.5 million 3D human keypoints annotations with eight subjects. They design a hardware-based sync calibration system with 10 RGB-D sensors to obtain the data. 
Several datasets include other emerging sensing modalities such as IMU~\cite{PonBaa2010a, vonPon2016a, vonMarcard2018} and mmWave signals\cite{zhao2018rf, an2021mars, sengupta2020mm, xue2021mmmesh} in human pose estimation task. They employ novel sensing modalities to capture the whole human body information and still use RGB or depth frame to obtain the human poses' ground truth. However, no HPE dataset currently combines intrusive and non-intrusive sensing modalities, including RGB/D, IMU, and mmWave signals.

% thesis statement: HPE in healthcare, it needs mmWave
% health datasets
% AHA-3D~\cite{antunes2018aha}
% UI-PRMD~\cite{vakanski2018data}
% Reiss et al.~\cite{reiss2012creating}
% EmoPain~\cite{aung2015automatic}
% HPTE~\cite{ar2014computerized}

\statement{Human pose estimation has played an increasingly crucial role in healthcare applications such as remote rehabilitation training.} Multiple datasets~\cite{antunes2018aha, vakanski2018data, reiss2012creating, ar2014computerized} have made a significant effort in combining HPE with health-related physical movements. The current mainstream rehabilitation treatment involves a physical therapist supervising the patients in person. HPE-based health monitoring systems can help clinicians correct patients' movements or instruct them remotely. Due to the particularity of healthcare application, ideally, HPE applied in it needs to be \textit{privacy-preserving}. For instance, patients often feel awkward and uncomfortable if their facial information is shown. It is critical to include privacy-preserving sensing modalities from both the non-intrusive side like mmWave and the intrusive side like IMUs for remote health monitoring development.

% 8000*20
% 30000*6*20
% 8000*20*6
In this work, we propose \textbf{\textit{mRI}}, a comprehensive 3D human pose estimation dataset performed by 20 human subjects, consisting of more than 5M frames from multiple sensing modalities. \textbf{\textit{mRI}} has the following major features:

\noindent{\textbf{Multiple Sensing Modalities.}}
\textbf{\textit{mRI}} consists of RGB frames, depth frames, inertial signals, and mmWave point cloud. The experiment captures the data by utilizing the following devices: two depth cameras, six high-accuracy inertial sensors~(IMUs), a commercial low-power, and a low-cost mmWave radar. Note that all sensors are temporally synchronized and spatially calibrated.

\noindent{\textbf{Healthcare Movements Focused.}}
We choose ten rehabilitation-specific movements suggested by clinicians. Specifically, these movements involve the upper body, lower body, and the major muscles related to human mobility. These movements are crucial for patients to recover from sequelae of central nervous system disorders, such as Parkinson's disease (PD) and cerebrovascular diseases (e.g., stroke).

\noindent{\textbf{Multiple Benchmarks.}}
We offer a comprehensive set of baseline and benchmarks for 2D/3D human pose estimation and action segmentation from multiple modalities. The proposed pipeline pre-processes all raw data into the point cloud, features, and 2D/3D keypoints. In addition, all manually-labeled actions annotations and 3D human key points ground truth are provided.

\noindent{\textbf{Low-power \& Low-cost.}}
\textbf{\textit{mRI}} focuses on practical indoor personalized rehabilitation system. To this end, all selected Internet-of-Things~(IoT) devices are low-power and low-cost. We envision sustainable, real-time HPE with all modalities using these sensors.
